Completely random measures for modelling block-structured networks

Many statistical methods for network data parameterize the edge-probability by attributing latent traits to the vertices such as block structure and assume exchangeability in the sense of the Aldous-Hoover representation theorem. Empirical studies of networks indicate that many real-world networks have a power-law distribution of the vertices which in turn implies the number of edges scale slower than quadratically in the number of vertices. These assumptions are fundamentally irreconcilable as the Aldous-Hoover theorem implies quadratic scaling of the number of edges. Recently Caron and Fox (2014) proposed the use of a different notion of exchangeability due to Kallenberg (2009) and obtained a network model which admits power-law behaviour while retaining desirable statistical properties, however this model does not capture latent vertex traits such as block-structure. In this work we re-introduce the use of block-structure for network models obeying Kallenberg's notion of exchangeability and thereby obtain a model which admits the inference of block-structure and edge inhomogeneity. We derive a simple expression for the likelihood and an efficient sampling method. The obtained model is not significantly more difficult to implement than existing approaches to block-modelling and performs well on real network datasets.

==> tex_images.tex <==
{% extends "arxiv1/index_partial.tex" %}
{% block figure7%}
\includegraphics[width=\linewidth]{figure7}{% endblock %}
{% block figure6%}
\includegraphics[width=\linewidth]{figure6}{% endblock %}
{% block figure3%} %EPPF_sampler_plotA
\includegraphics[width=\linewidth]{figure3}{% endblock %}
{% block figure1%}
\includegraphics[width=\linewidth]{figure1}{% endblock %}
{% block figure101%}
\includegraphics[width=\linewidth]{figure101}{% endblock %}
{% block figure11%}
\includegraphics[width=.8\linewidth]{figure11}{% endblock %}
{% block figure10%}
\includegraphics[width=.8\linewidth]{figure10}{% endblock %}
{% block figure9%}
\includegraphics[width=\linewidth]{figure9}{% endblock %}
{% block figure8%}
\includegraphics[width=\linewidth]{figure8}{% endblock %}
